Analysis of t tbar H Events at sqrt(s)=14 TeV with H -> WW

We study the process pp -> t tbar H at sqrt(s)=14 TeV where H -> WW. We focus on final states that include three or four leptons. Signal and background samples are generated at leading order (LO) and normalized to next-to-leading order (NLO) calculations. We employ the "Snowmass" detector simulation and event reconstruction. Cuts are selected which provide a substantial signal yield while suppressing the main backgrounds. Systematic uncertainties are estimated for the overall normalization of signal and background processes. With no improvement in the current theoretical uncertainties on sigma(t tbar H), we project a precision on a top quark Yukawa coupling of approximately 16% in 300 fb^-1 and 9% in 3000 fb^-1. If the theoretical uncertainties are halved, these improve to 14% and 6%, respectively.

==> Makefile <==
ATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = Theory 

default: internaldraft 
#default: public

internaldraft:
	pdflatex  '\newcommand{\extramaterial}{true}\newcommand{\draft}{true}\input{${BASENAME}}'
	pdflatex  '\newcommand{\extramaterial}{true}\newcommand{\draft}{true}\input{${BASENAME}}'
	bibtex bu1 
	pdflatex  '\newcommand{\extramaterial}{true}\newcommand{\draft}{true}\input{${BASENAME}}'
	pdflatex  '\newcommand{\extramaterial}{true}\newcommand{\draft}{true}\input{${BASENAME}}'

public:
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{false}\input{${BASENAME}}'
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{false}\input{${BASENAME}}'
	bibtex bu1			                      
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{false}\input{${BASENAME}}'
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{false}\input{${BASENAME}}'
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

publicdraft:
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{true}\input{${BASENAME}}'
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{true}\input{${BASENAME}}'
	bibtex bu1
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{true}\input{${BASENAME}}'
	latex  '\newcommand{\extramaterial}{false}\newcommand{\draft}{true}\input{${BASENAME}}'
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 



